Low-Complexity High-Performance Cyclic Caching for Large MISO Systems

Multi-antenna coded caching is known to combine a global caching gain that is proportional to the cumulative cache size found across the network, with an additional spatial multiplexing gain that stems from using multiple transmitting antennas. However, a closer look reveals two severe bottlenecks; the well-known exponential subpacketization bottleneck that dramatically reduces performance when the communicated file sizes are finite, and the considerable optimization complexity of beamforming multicast messages when the SNR is finite. We here present an entirely novel caching scheme, termed \emph{cyclic multi-antenna coded caching}, whose unique structure allows for the resolution of the above bottlenecks in the crucial regime of many transmit antennas. For this regime, where the multiplexing gain can exceed the coding gain, our new algorithm is the first to achieve the exact one-shot linear optimal DoF with a subpacketization complexity that scales only linearly with the number of users, and the first to benefit from a multicasting structure that allows for exploiting uplink-downlink duality in order to yield optimized beamformers ultra-fast. In the end, our novel solution provides excellent performance for networks with finite SNR, finite file sizes, and many users.

==> BACKUPLinearSubpacks.tex <==
In this section, we present our low-complexity high performance cyclic caching scheme, which can be applied to any MISO setup in which $\alpha \ge t$.\footnote{For setups with $t > \alpha$, one can use the coded caching scheme presented in~\cite{lampiris2018adding} for reduced subpacketization.} 
%We first provide the mathematical representation of a basic scheme that requires subpacketization of $K(t+\alpha)$ to achieve the sum DoF of $t+\alpha$. Next, we clarify the procedure of the proposed scheme with the help of an illustrative graphical example. Finally, we use a user-grouping approach to modify the basic scheme in order to further reduce the required subpacketization by a factor of $\phi_{K,t,\alpha}^2$, where $\phi_{K,t,\alpha} = gcd(K,t,\alpha)$. 
The following theorem summarizes the contribution of this paper:
\begin{thm}
\label{thm:main_contribution}
For the cache-aided MISO setup considered in this paper, for which $t \le \alpha \le L$, the sum DoF of $t+\alpha$ is achievable with a subpacketization requirement of only
\begin{equation}
\label{eq:min_subpack}
    \frac{K(t+\alpha)}{\phi_{K,t,\alpha}^2}.
\end{equation}
\end{thm}
\begin{proof}
The cyclic caching scheme, presented in this section, achieves the sum DoF of $t+\alpha$ with the proposed subpacketization. Specifically, we first introduce a cache placement algorithm in Section~\ref{section:lin_placement}, which is based on a well-defined placement matrix and requires each file to be split into $K(t+\alpha)$ smaller parts (subpackets). In Sections~\ref{section:lin_delivery} and~\ref{section:lin_decoding}, we explain the delivery phase, in which the missing data parts are delivered to the requesting users with the help of $K(K-t)$ multicast transmission vectors, each serving $t+\alpha$ subpackets to $t+\alpha$ different users. In Section~\ref{section:graphical_rep}, we show that this delivery algorithm follows a simple graphical representation, involving circular shifting of two vectors over a tabular structure. Overall, in Sections~\ref{section:lin_placement} to~\ref{section:graphical_rep}, we present a scheme which satisfies all the requests with multicast transmissions always containing $t+\alpha$ subpackets
; it follows that the scheme achieves a sum DoF of $t+\alpha$ with a subpacketization requirement of $K(t+\alpha)$, which is the same value as the nominator of~\eqref{eq:min_subpack}.

Following the discussions in Sections~\ref{section:lin_placement} to~\ref{section:graphical_rep}, in Section~\ref{section:Emanuele_part}, we show that the subpacketization requirement can be further reduced by a factor of $\phi_{K,t,\alpha}^2$, without any loss in the achievable sum DoF. This reduction is possible with a user grouping technique, which enables the original network to be mapped into a smaller \textit{virtual} network. We show that applying the coded caching scheme presented in Sections~\ref{section:lin_placement} to~\ref{section:graphical_rep} to the virtual network, and then \textit{elevating} the resulting cache placement and delivery procedures to be applicable to the original network, it is possible to reduce the required subpacketization by a factor of $\phi_{K,t,\alpha}^2$, without losing the achievable sum DoF. The reduction factor of $\phi_{K,t,\alpha}^2$ is the same value in the denominator of~\eqref{eq:min_subpack}, and hence, this completes the proof.
%The scheme achieving the optimal sum DoF with the reduced subpacketization stated in the theorem is presented later in this section, and the optimality of the achievable DoF can be proved by means of the lower bound in \cite{lampiris2018resolving}.
\end{proof}

\begin{rem}
\label{rem:optimal_dof}
If $\alpha=L$, the proposed scheme achieves the \textit{optimal} sum DoF of $t+L$ with a subpacketization requirement of $\frac{K(t+L)}{\phi_{K,t,L}^2}$. The exact optimality of $t+L$ in the one-shot linear sum DoF sense is shown in~\cite{lampiris2018resolving}.
\end{rem}

%Theorem~\ref{thm:main_contribution} follows directly from the novel cache placement and content delivery algorithms presented in Sections~\ref{section:lin_placement}, \ref{section:lin_delivery}, and~\ref{section:Emanuele_part}. 
According to the definition of the greatest common divisor, all the three parameters $K$, $t$ and $\alpha$ are divisible by $\phi_{K,t,\alpha}$, and hence, the subpacketization value in~\eqref{eq:min_subpack} is an integer. Moreover, from~\eqref{eq:min_subpack} it is clear that for a fixed $t$ value, the subpacketization requirement of the  cyclic caching scheme scales linearly with the number of users $K$.\footnote{If $t$ scales with $K$, the growth is quadratic, which is still much less than the exponential growth of other well-known schemes such as~\cite{shariatpanahi2018physical}.} The result is a high-performance, low-subpacketization scheme, which is nicely applicable to large networks. A smaller subpacketization also generally implies a smaller number of transmissions, thus reducing the number of beamformer design problems to be solved. As a quick comparison, consider a moderate-sized network of $K=20$ users, in which the transmitter is equipped with $L=8$ antennas and the coded caching gain is $t=4$. Assuming the antenna array is used to achieve the maximum spatial multiplexing gain of $\alpha=8$, our scheme achieves the optimal sum DoF of $4+8=12$ with a subpacketization requirement of 15. In comparison, the subpacketization requirement for the original multi-antenna scheme in~\cite{shariatpanahi2018physical} is larger than $3 \times 10^7$; and for the recent scheme in~\cite{mohajer2020miso} it is 4845. More detailed comparison results are provided in Section~\ref{section:sim_results}.

\subsection{Cache Placement}
\label{section:lin_placement}
For cache placement, we use a placement matrix $\BV$, which is a $K \times K$ binary matrix in which the first row has $t$ consecutive one elements (other elements are zero) and for the other rows, each row is a circular shift of the previous row by one unit. Given $\BV$, we split each file $W$ into $K$ smaller parts $W_p$, $p \in [K]$, and each part $W_p$ into $t+\alpha$ smaller parts $W_p^q$. Then for every $p,k\in [K]$, if $\BV[p,k] = 1$, $W_p^q$ is stored in the cache memory of user $k$, $\forall W \in \CF, q \in [t+\alpha]$. For the sake of simplicity, we use the term \textit{packet} to refer to $W_p$, and \textit{subpacket} to refer to $W_p^q$, for some general $W \in \CF$, $p \in [K]$ and $q \in [t+\alpha]$.\footnote{The placement matrix $\BV$ used in this paper is a special case of valid placement matrices introduced in~\cite{salehi2019subpacketization}.}

\begin{exmp}
\label{exmp:placement_matrix}
Assume $K=6$, $t=2$, $\alpha=3$. $\BV$ is built as
\begin{equation}
\BV = 
    \begin{bmatrix}
    1 & 1 & 0 & 0 & 0 & 0 \\
    0 & 1 & 1 & 0 & 0 & 0 \\
    0 & 0 & 1 & 1 & 0 & 0 \\
    0 & 0 & 0 & 1 & 1 & 0 \\
    0 & 0 & 0 & 0 & 1 & 1 \\
    1 & 0 & 0 & 0 & 0& 1
    \end{bmatrix} \; ,
\end{equation}
and subpacketization is $K \times (t+\alpha) = 6 \times (2+3) = 30$.
%If $\CF = \{ A,B,C,D,E,F \}$, we have
The cache contents of user 1 and 2 are
\begin{equation*}
    \begin{aligned}
    \CZ(1) = &\{ W_1^q, W_6^q \; ; \; \forall \, W \in \CF , \, q\in[5] \} \; , \\
    \CZ(2) = &\{ W_1^q, W_2^q \; ; \; \forall \, W \in \CF , \, q\in[5] \} \; . \\
    %&W_6^1, W_6^2, W_6^3, W_6^4, W_6^5 \; \mid \; W \in \CF\} \; ,
    %\CZ(1) = \{ &W_1^1, W_1^2, W_1^3, W_1^4, W_1^5, W_6^1, W_6^2, W_6^3, W_6^4, W_6^5, B_6^2, B_6^3, \\
    %&C_1^1, C_1^2, C_1^3, C_6^1, C_6^2, C_6^3, D_1^1, D_1^2, D_1^3, D_6^1, D_6^2, D_6^3,\\
    %&E_1^1, E_1^2, E_1^3, E_6^1, E_6^2, E_6^3, F_1^1, F_1^2, F_1^3, F_6^1, F_6^2, F_6^3 \} \; .
    \end{aligned}
\end{equation*}
The cache content of other users can be written accordingly.
\end{exmp}

\input{LinearS-Delivery}



==> Data/K-Change.tex <==
t	L	K	ChannelRate	TotalRate
2	4	8	6.6342	8.8456
2	4	9	6.5703	8.447528571
2	4	10	6.3336	7.917
2	4	11	6.4649	7.901544444
2	4	12	6.4619	7.75428
2	4	13	6.3764	7.535745455
2	4	14	6.6347	7.740483333
2	4	15	6.4968	7.496307692
2	4	16	6.4195	7.336571429
2	4	17	6.3513	7.19814
2	4	18	6.213	6.989625
2	4	19	6.2807	7.019605882
2	4	20	6.4038	7.115333333
2	4	21	6.2861	6.947794737
2	4	22	6.4865	7.13515
2	4	23	6.4319	7.044461905
2	4	24	6.3263	6.901418182
2	4	25	6.5544	7.124347826
2	4	26	6.4682	7.007216667
2	4	27	6.3413	6.848604
2	4	28	6.4818	6.9804
2	4	29	6.2868	6.752488889
2	4	30	6.4152	6.873428571


==> Data/L-Change.tex <==
t	L	K	ChannelRate	TotalRate
2	4	30	6.3224	6.774
2	5	30	7.8342	8.393785714
2	6	30	9.0412	9.687
2	7	30	10.5061	11.25653571
2	8	30	11.8659	12.71346429
2	9	30	12.932	13.85571429
2	10	30	14.2968	15.318
2	11	30	15.6428	16.76014286
2	12	30	16.9704	18.18257143
2	13	30	18.2721	19.57725
2	14	30	19.4463	20.83532143
2	15	30	20.8526	22.34207143
2	16	30	22.2079	23.79417857
2	17	30	23.5548	25.23728571
2	18	30	24.7704	26.53971429
2	19	30	26.2821	28.15939286
2	20	30	27.2727	29.22075
2	21	30	28.9525	31.02053571
2	22	30	30.0046	32.14778571
2	23	30	31.198	33.42642857
2	24	30	32.6594	34.99221429


==> Data/SN1-3-Rate.tex <==
SNR	MS-A1	MS-A2	MS-A3	LIN-A2	LIN-A3	NOC-A1	NOC-A2	NOC-A3	RED-A2	Bound-A1	Bound-A2	Bound-A3
-5	1.429215518	1.452	1.48425	0.91335	0.9279	0.52857695	0.5472	0.56865	0.9132	1.236464516	1.648619354	2.060774193
0	3.499826839	3.625244809	3.518957382	2.318417246	2.202688224	1.16500118	1.258224791	1.247566623	2.317795278	3.119162313	4.158883083	5.198603854
5	6.948345185	7.41207936	7.173119714	4.930079412	4.498279916	2.087778436	2.431982147	2.365555867	4.934163633	6.417280975	8.556374633	10.69546829
10	11.4202789	12.68719749	12.22095239	8.938072235	7.689637876	3.171318939	4.075590255	3.891739846	8.967220569	10.79052873	14.38737164	17.98421455
15	16.38189554	19.01335079	18.63236411	14.30101336	11.83398565	4.313712505	6.090540591	5.897240243	14.35744158	15.68254821	20.91006428	26.13758035
20	21.5159874	25.84052079	26.26703334	20.58331178	17.18166352	5.471320938	8.310705007	8.4292547	20.64361661	20.76804233	27.6907231	34.61340388
25	26.69909038	32.81056517	34.74285708	27.31756809	23.78754592	6.630907483	10.60979252	11.41115982	27.37501732	25.91829009	34.55772012	43.19715015
30	31.89173018	39.78548244	43.62716879	34.18926681	32.34285887	7.789388326	12.92924651	15.00757644	34.2336021	31.08939651	41.45252868	51.81566084


==> Data/SN4-6-L25-Rate.tex <==
SNR	RED-A10	RED-A15	RED-A20	NOC-A10	NOC-A15	NOC-A20	RED15-10	RED20-10	NOC15-10	NOC20-10
-5	6.569888889	6.576777778	6.576666667	5.001222222	5.261444444	5.399444444	0 	0 	5 	8 
0	15.16421973	15.16164676	15.08767918	10.37121161	11.20453846	11.58849548	0 	-1 	8 	12 
5	29.36893722	29.36685508	28.82029088	18.25475684	20.28234539	20.90530347	0 	-2 	11 	15 
10	48.82054586	49.43607392	47.62402803	28.07938455	32.48271211	33.23356595	1 	-2 	16 	18 
15	71.80055092	74.88163098	71.5636454	38.95480377	47.26699209	48.74725167	4 	0 	21 	25 
20	96.45402856	104.0466958	100.9594729	50.2543831	63.56639141	67.51802067	8 	5 	26 	34 
25	121.732778	135.0149648	134.9913768	61.70017988	80.50754776	88.69307745	11 	11 	30 	44 
30	147.2206597	166.6639379	171.6923122	73.19310547	97.6740669	111.0626673	13 	17 	33 	52 
35

==> Data/SN7-8-K100-Rate.tex <==
SNR	RED-KF0	RED-KF5	RED5-0
-5	5.004731183	4.836344086	-3 
0	11.47412876	11.24926715	-2 
5	21.98235535	21.60080635	-2 
10	36.65520626	35.98645738	-2 
15	55.53002059	54.34283902	-2 
20	77.9958151	75.97099917	-3 
25	102.604986	99.48942666	-3 
30	128.1320568	123.7954149	-3
35

==> Data/SN7-8-K30-Rate.tex <==
SNR	RED-KF0	RED-KF5	RED5-0	NOC-KF0	NOC-KF5	NOC5-0
-5	6.082043478	5.262130435	-13 	4.248782609	3.967434783	-7 
0	13.91823859	12.67506307	-9 	9.111414252	8.767071847	-4 
5	26.65890912	24.45981524	-8 	16.52475738	15.97860039	-3 
10	44.45286137	40.65499249	-9 	26.54417208	25.55160427	-4 
15	67.34234014	60.92538655	-10 	39.12684805	37.16297385	-5 
20	94.58463275	84.26381923	-11 	53.65588992	50.11114999	-7 
25	124.4276269	109.2517976	-12 	69.19460059	63.6736291	-8 
30	155.3867909	134.8944514	-13 	85.12641763	77.44871983	-9 
35

==> Intro.tex <==
Wireless networks play a significant role in our life nowadays and are also a key enabler for interesting futuristic applications such as wireless immersive viewing and reliable autonomous driving. Every new application puts tighter restrictions on various networking KPIs (key performance indicators) such as the data rate, delay, and reliability. Among these KPIs, the achievable data rate has always been of significant importance, mainly due to the unprecedented dominance of multimedia applications~\cite{cisco2018cisco}.  Coded caching, proposed by Maddah-Ali and Niesen in~\cite{maddah2014fundamental}, is considered as a promising option for increasing the data rate. In a network of cache-enabled users in which the users can pre-fetch data into their cache memories, coded caching enables the achievable rate to be increased (or the required bandwidth to be decreased) in proportion to the total cache size in the network. This speed-up factor, known as coded caching gain, is enabled by multicasting carefully created codewords to different subsets of users, such that each user in the target set can use its cache content to remove unwanted terms from the received codeword. Interestingly, in a wireless communication setup with $L$ transmitting antennas, the coded caching gain is additive with the spatial multiplexing gain; i.e., the speed-up factor of $t+L$ is achievable, where $t$ is the coded caching gain~\cite{shariatpanahi2016multi,shariatpanahi2018physical}. This property makes coded caching an even more desirable technique, as multi-input multi-output (MIMO) communication is expected to play a significant role in future wireless networks~\cite{rajatheva2020white}.

However, despite the original theoretical promises for the substantial caching gains that scale with the available cache storage throughout the network, in reality, coded caching schemes suffer from severe fundamental implementation bottlenecks.
One of the most impactful bottlenecks is the large subpacketization requirement, where subpacketization is the number of smaller parts each file is split into, for a coded caching scheme to work correctly. 
The original coded caching scheme in~\cite{maddah2014fundamental} requires a subpacketization value that grows exponentially with the number of users in the network, which means the size of each file (and respectively, each cache) should also grow exponentially with the user count. This issue makes the implementation infeasible, even for moderate-sized networks. The problem is more severe for the baseline multi-antenna coded caching scheme of~\cite{shariatpanahi2018physical}, as its subpacketization requirement is a multiplicative factor of the original scheme in~\cite{maddah2014fundamental}, and the multiplier itself grows exponentially with the network size. 

Recent breakthroughs have shown that with the help of multi-antenna transmitting arrays, it is possible to dramatically improve the subpacketization bottleneck. Interestingly, for a large selection of network parameters, the subpacketization requirement of a multi-antenna setup can even be smaller than a single-antenna counterpart~\cite{lampiris2018adding}. This property reveals the prominent role of multi-antenna transmissions, not only for providing the spatial multiplexing gain on top of the coded caching gain but also for reducing the subpacketization requirement in large networks. However, the novel algorithms in~\cite{lampiris2018adding} apply in their full optimality only for networks in which the spatial multiplexing gain $L$ does not exceed the coded caching gain $t$. Thus it remains an open question to investigate whether it is possible to design a multi-antenna coded caching scheme with optimal DoF (degrees of freedom) for networks with large antenna arrays in which $L \ge t$. Moreover, in~\cite{lampiris2018adding} the authors only consider the high-SNR (signal to noise ratio) communication regime. Although the high-SNR analysis is useful for investigating the achievable DoF and establishing performance bounds, for real-world implementation, one needs efficient schemes with moderate implementation complexity at the low- and mid-SNR communication regimes.

%I moved these to the end of new/merged introduction

% In this paper, we introduce an entirely new DoF-optimal low-subpacketization coded caching scheme, applicable to networks with large transmitting antenna arrays, in which the spatial multiplexing gain is larger than or equal to the coded caching gain. The proposed scheme not only requires much smaller subpacketization values compared with the state of the art but also benefits from an underlying cache-aided interference cancellation mechanism that enables efficient optimized MMSE (minimum min-square error) type beamformers to be applied with low computational complexity. This enables the performance of the proposed scheme to be superior at the low- and mid-SNR regime, compared with the case zero-forcing beamformers are used to completely remove the inter-stream interference. In other words, our scheme enables an interplay between cache cancellation and interference suppression, which results in a highly efficient low-subpacketization coded caching scheme with an appropriate performance at the finite-SNR regime.


% In this paper, we use $[K]$ to denote  $\{1,2,...,K\}$ and $[i:j]$ to represent $\{i,i+1,...,j\}$. Boldface upper- and lower-case letters denote matrices and vectors, respectively. $\BV[i,j]$ refers to the element at the $i$-th row and $j$-th column of matrix $\BV$, and $\Bw[i]$ is the $i$-th element in vector $\Bw$. Sets are denoted by calligraphic letters. For two sets $\CA$ and $\CB$, $\CA \backslash \CB$ is the set of elements in $\CA$ which are not in $\CB$; and $|\CA|$ represents the number of elements in $\CA$.


==> LargerArrays.tex <==
In this section we will discuss how extra antennas can be used for beamformer enhancement. The case with $L+t > K$ will be considered, and an effective antenna count $L'$ will be selected such that subpacketization is reduced considerably (Emanuele's extension). The remaining antennas will then be used for beamformer enhancement.

Side idea: if $L' = k-t$, flexible subpacketization also becomes possible, according to our Globecom paper.

==> LinearS-Delivery-Old.tex <==
------------------------------------------------------

\textbf{This is the old text}

%This can be made simpler by introduction of auxiliary variables. We can introduce transmission round $r$ and round index $j$. Then for each index at each round, we build a transmission vector. The targeted user set $\CR(r,j)$ and subpacket index set $\CC(r,j)$ can be defined recursively. First, $\CR(1,j)$ is built based on $\CR(1,1)$; and then $\CR(r,j)$ is built from $\CR(1,j)$. Another option to assume these sets are vectors; and then denote their $i$-th element with $\Br_r(j)$, for example. Overall, the introduction of rounds and round indices is a good idea I think. 

Consider the generic transmitted vector
\begin{equation}
\mathbf{x}(S)=\sum_{j\in S}\mathbf{w}_{\mathcal{T}_j}X_j,
\end{equation}
where $\mathbf{w}_{\mathcal{T}_j}$ denotes the general beamformer vector for message $X_j$.
We define \textit{$k$-shifted vector} of $\mathbf{x}(S)$ the vector
\begin{equation}\label{eq:shift}
\mathbf{x}^{(k)}(S)=\sum_{j\in S}\mathbf{w}_{\mathcal{T}^{(k)}_j}X_{(j+k)\%K},
\end{equation}
where $\mathcal{T}^{(k)}_j$ is the set obtained by adding (modulo $K$) $k$ units to each element in $\mathcal{T}_j$, i.e.
$$\mathcal{T}^{(k)}_j=\{(\mathcal{T}_j(i)+k)\%K~|~\forall i\in [|\mathcal{T}_j|]\}.$$ 

The delivery phase is comprised of $K$ rounds, each, in turn, consisting of $K-t$ transmissions. The transmissions in the first round take the form  
\begin{align}
&\mathbf{x}_i=\sum_{j\in[t]}\mathbf{v}^{\perp}_{\mathcal{R}_{i,j}}W^{l}_{(t+1+i)\%K}(j)+\sum_{j\in[(t+1+i)\%K:(t+L+i)\%K]}\mathbf{v}^{\perp}_{\mathcal{P}_{i,j}}W^{l}_1(j) ~~~\forall i \in\{0,1,\dots,K-t-1\}\\
&\text{where} ~~ 
\mathcal{R}_{i,j}=[t]\setminus\{j\} \cup [(2t+i)\%K:(t+L+i)\%K]\\ 
&\text{and} ~ ~ \mathcal{P}_{i,j}=[(t+1+i)\%K:(t+L+i)\%K]\setminus\{j\},
\end{align}
and where $l$ is an index chosen sequentially, and independently for each subfile $W_p(j)$, from the set $[t+L]$.
Each of the remaining rounds $r\in[K-1]$ consists of $K-t$ transmissions obtained by $r$-shifting the transmitted vectors of the first round as in in  \eqref{eq:shift}, i.e. the $K-t$ transmissions of round $r$ are
\begin{equation}
\mathbf{x}_i^{(r)} ~~~ \forall i\in\{0,1,\dots,K-t-1\},
\end{equation}
where $\mathbf{x}_i^{(r)}$ is the \textit{r-shifted vector} of $\mathbf{x}_i$.

\subsection{Algorithmic Representation}

\textbf{Delivery Prime Matrices}

\label{section:delivery_prime_matrix}
In order to provide the delivery algorithm, we first introduce and construct Delivery Prime (DP) matrices. Denoted by $\BR_k$ and $\BC_k$, $k \in [K]$, they are a group of matrices with dimensions $(K-t) \times (t+L)$. $\BR_1$ and $\BC_1$ are built using Algorithms \ref{alg:R1_creation} and \ref{alg:C1_creation} (for all algorithms, $K, L, N, t$ are assumed to be global variables known to the procedures);
%\footnote{For all algorithms, $K$, $L$, $N$ and $t$ are assumed to be global variables known to the procedures}; 
%and for $k>1$, $\BR_k$ and $\BC_k$ are built from $\BR_{k-1}$ and $\BC_{k-1}$, respectively.
and for $k > 1$, we use circular increment to build $\BR_k$ and $\BC_k$ from $\BR_{k-1}$ and $\BC_{k-1}$, respectively. For an integer $a$, the intended circular increment operation in domain $K$ is defined as
\begin{equation}
    i_c (a,K) = (a \mod K) + 1 \; ,
\end{equation}
while for a matrix $\BA$ with positive integer elements, $i_c(\BA,K)$ results in a matrix in which each element is the circular increment (in domain $K$) of its respective element in $\BA$. Now for $k \in [2:K]$ we define
\begin{equation}
    \begin{aligned}
    \BR_k = i_c(\BR_{k-1},K) \; ; \;\; \BC_k = i_c(\BC_{k-1},K) \; .
    \end{aligned}
\end{equation}
%
%The generator procedures for $\BR_1$ and $\BC_1$ are described by Algorithms \ref{alg:R1_creation} and \ref{alg:C1_creation}, respectively (note that for all algorithms in this paper, $K$, $L$, $N$ and $t$ are assumed to be global variables known to the procedures).
\begin{exmp}
\label{exmp:r1_c1}
For the network of Example \ref{exmp:placement_matrix}, we have
\begin{equation}
\label{eq:r1_exmp_1}
\begin{aligned}
    \BR_1 =
    \begin{bmatrix}
    3 & 3 & 1 & 1 & 1 \\
    4 & 4 & 1 & 1 & 1 \\
    5 & 5 & 1 & 1 & 1 \\
    2 & 6 & 1 & 1 & 1
    \end{bmatrix}, 
    \; \BC_1 =
    \begin{bmatrix}
    1 & 2 & 3 & 4 & 5 \\
    1 & 2 & 4 & 5 & 6 \\
    1 & 2 & 5 & 6 & 3 \\
    1 & 2 & 6 & 3 & 4
    \end{bmatrix}, \\
    \BR_2 =
    \begin{bmatrix}
    4 & 4 & 2 & 2 & 2 \\
    5 & 5 & 2 & 2 & 2 \\
    6 & 6 & 2 & 2 & 2 \\
    3 & 1 & 2 & 2 & 2
    \end{bmatrix},
    \; \BC_2 =
    \begin{bmatrix}
    2 & 3 & 4 & 5 & 6 \\
    2 & 3 & 5 & 6 & 1 \\
    2 & 3 & 6 & 1 & 4 \\
    2 & 3 & 1 & 4 & 5
    \end{bmatrix}.
\end{aligned}
\end{equation}
\end{exmp}


\begin{algorithm}[t]
\caption{$\BR_1$ Generation Procedure}
\label{alg:R1_creation}
\begin{algorithmic}[1]
    \Procedure{Generate $\BR_1$}{}
        \ForAll{$j \in [1:t]$}
            \ForAll{$i \in [1:K-2t+j]$}
                \State $\BR_1 [i,j] \gets t+i$
            \EndFor
            \ForAll{$i \in [K-2t+j+1:K-t]$}
                \State $\BR_1 [i,j] \gets t+i-(K-2t+j-1)-t$
            \EndFor
        \EndFor
        \ForAll{$j \in [t+1:t+L]$, $i \in [1:K-t]$}
            \State $\BR_1 [i,j] \gets 1$
        \EndFor
    \EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{$\BC_1$ Generation Procedure}
\label{alg:C1_creation}
\begin{algorithmic}[1]
    \Procedure{Generate $\BC_1$}{}
        \ForAll{$j \in [1:t]$, $i \in [1:K-t]$}
            \State $\BC_1 [i,j] \gets j$
        \EndFor
        \ForAll{$j \in [t+1:t+L]$, $i \in [1:K-t]$}
            \If{$j+i-1 \le K$}
                \State $\BC_1 [i,j] \gets j+i-1$
            \Else
                \State $\BC_1 [i,j] \gets j+i-1-(K-t)$
            \EndIf
        \EndFor
    \EndProcedure
\end{algorithmic}
\end{algorithm}

\textbf{The Delivery Algorithm}

Delivery procedure is provided in Algorithm \ref{alg:delivery_main}; with its auxiliary procedures presented in Algorithms \ref{alg:aux_init} and \ref{alg:aux_gen_r}. We have used $\{ \BC_k \} \equiv \{ \BC_1, ..., \BC_K \}$ and $\{ \BR_k \} \equiv \{ \BR_1, ..., \BR_K \}$; and \textsc{Modulate} function returns the modulated version of its input.
The procedure is based on DP matrices. For each $k \in [K]$ we use $\BR_k$ and $\BC_k$ jointly, to create one transmission round. Each round has $K-t$ transmission vectors; resulting in $S = K \times (K-t)$ transmission intervals in total.

% Delivery procedure is provided through Algorithms~\ref{alg:delivery_main}-\ref{alg:aux_gen_r}, where $\{ \BC_k \} \equiv \{ \BC_1, \BC_2, ..., \BC_K \}$ and $\{ \BR_k \} \equiv \{ \BR_1, \BR_2, ..., \BR_K \}$
%\begin{equation*}
%    \begin{aligned}
%        \{ \BC_k \} &\equiv \{ \BC_1, \BC_2, ..., \BC_K \} , \\
%        \{ \BR_k \} &\equiv \{ \BR_1, \BR_2, ..., \BR_K \} ,
%    \end{aligned}
%\end{equation*}
%and \textsc{Modulate} function returns the modulated version of its input.

As an explanation, for every $k \in [K]$, a transmission~vector $\Bx(s)$ is built for each row in $\BR_k$ and $\BC_k$. More precisely, the entries in each row of $\BC_k$ specify the user indices to be targeted during the transmission interval, i.e. $\CT(s)$; while the entries in the respective row of $\BR_k$ clarify the file parts to be selected for users in $\CT(s)$. Finally, for $n \in [N]$, $k \in [K]$, the superscript $q(n,k)$ is another index which exactly specifies which data portion should be sent during each transmission.

%\begin{exmp}
%\label{exmp:trans_vectors_exmp}
%Consider the same network of Example \ref{exmp:r1_c1}.
%Consider a network with $K = 6, t = 2, L = 3$; for which $\BR_1, \BC_1$ are provided in \eqref{eq:r1_exmp_1}. 
%For demand set $\CD = \{A,B,C,D,E,F \}$, the transmission vectors of the first round include (modulation effect is ignored for notation simplicity):
%\begin{equation}
%    \begin{aligned}
%        \Bx(1) = &A_3^1 \Bv_{\{1,3,4\}} + B_3^1 \Bv_{\{2,3,4\}} \\
%            &+ C_1^1 \Bv_{\{1,2,3\}} + D_1^1 \Bv_{\{1,2,4\}} + E_1^1 \Bv_{\{1,2,5\}} \; , \\
%        \Bx(2) = &A_4^1 \Bv_{\{1,4,5\}} + B_4^1 \Bv_{\{2,4,5\}} \\
%            &+ D_1^2 \Bv_{\{1,2,4\}} + E_1^2 \Bv_{\{1,2,5\}} + F_1^1 \Bv_{\{1,2,6\}} \; , \\
%        \Bx(3) = &A_5^1 \Bv_{\{1,5,6\}} + B_5^1 \Bv_{\{2,5,6\}} \\
%            &+ E_1^3 \Bv_{\{1,2,5\}} + F_1^2 \Bv_{\{1,2,6\}} + C_1^2 \Bv_{\{1,2,3\}} \; , \\
%        \Bx(4) = &A_2^1 \Bv_{\{1,2,3\}} + B_6^1 \Bv_{\{1,2,6\}} \\
%            &+ F_1^3 \Bv_{\{1,2,6\}} + C_1^3 \Bv_{\{1,2,3\}} + D_1^3 \Bv_{\{1,2,4\}} \; ,
%    \end{aligned}
%\end{equation}
%Similarly, for each $k \in [2:6]$, there exist four transmission vectors in round $k$.
%\end{exmp}

\begin{algorithm}[t]
\caption{Delivery Procedure}
\label{alg:delivery_main}
\begin{algorithmic}[1]
    \Procedure{Delivery}{$\{\BR_k \}, \{\BC_k \}$}
        \State \textsc{Initialize}
        \ForAll{$k \in [K]$}
            \ForAll{$i \in [K-t]$}
                \State $s \gets s+1$
                \State $\Bx(s) \gets 0$
                \ForAll{$j \in [t+L]$}
                    \State $usr \gets \BC_k[i,j]$
                    \State $prt \gets \BR_k[i,j]$
                    \State $ind \gets q \big( W(usr),prt \big)$
                    \State $\SfX \gets $ \textsc{Modulate}$\big( W_{prt}^{ind} (usr) \big)$
                    \State $\CR \gets$ \textsc{Generate $\CR$}($k, i, usr, prt, \{\BC_k \}$)
                    \State $\Bx(s) \gets \Bx(s) + \Bv_{\CR} \SfX$
                    \State $q \big( W(usr),prt \big) \gets q \big( W(usr),prt \big) + 1$
                \EndFor
                \State Transmit $\Bx(s)$
            \EndFor
        \EndFor
    \EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{Initialization Procedure}
\label{alg:aux_init}
\begin{algorithmic}[1]
    \Procedure{Initialize}{}
        \State $s \gets 0$
        \ForAll{$n \in [N]$, $p \in [K]$}
            \State $q(n,p) \gets 1$
        \EndFor
    \EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{$\CR$ Generation Function}
\label{alg:aux_gen_r}
\begin{algorithmic}[1]
    \Function{Generate $\CR$}{$k, row, usr, prt, \{\BC_k\}$}
            \State $\CR \gets \{usr \}$
            \ForAll{$r \in [t+L]$}
                \State $node \gets \BC_k[row,r]$
                \If{$\BV[prt,node] = 1$}
                    \State $\CR \gets \CR \cup \{node \}$
                \EndIf
            \EndFor
            \State \Return $\CR$
    \EndFunction
\end{algorithmic}
\end{algorithm}

==> LinearS-Graphical.tex <==
\subsection{Graphical Representation}
\label{section:graphical_rep}
Before formal description of the delivery algorithm, we provide a graphical illustration of its operation for the network of Example \ref{exmp:placement_matrix}.
The delivery algorithm operates in $K=6$ rounds and at each round, $K-t=4$ transmission vectors are built; resulting in $S=24$ total transmission intervals. We also assume the demand set is $\CD = \{A,B,C,D,E,F\}$, and ignore the modulation effect for notation clarity.

Graphical illustration for the first and second rounds are provided in Figures
%This representation is provided in Figures
\ref{fig:graph_exmp_r1c1} and \ref{fig:graph_exmp_r2c2}, respectively. In both figures, each matrix column represents a user and each row stands for a file part index. For example, the first column represents user one, and the first row stands for the first part of all files; i.e. $W_1^q$, $\forall W \in \CF, q \in [t+L]$.
A lightly shaded entry in the matrix means the data part is cached at the respective user.~For example,
$W_1^q,W_6^q$ are stored at user 1, $\forall W \in \CF, q \in [t+L]$. Clearly, the cache placement indicated by Figures \ref{fig:graph_exmp_r1c1} and \ref{fig:graph_exmp_r2c2} is equivalent to the placement matrix $\BV$ provided in Example \ref{exmp:placement_matrix}. 
%the cell in the first row and first column of the grids is lightly shaded, which means $W_1^q$ is stored at the cache memory of user one, for every $W \in \CF$ and $q \in [t+L]$. It can be easily verified that the cache placement of Figures \ref{fig:graph_exmp_r1c1} and \ref{fig:graph_exmp_r2c2} matches the scheme of Section \ref{subsection:placement}.

Consequently, a dark shaded entry indicates which index of the requested file is sent to the respective user, during the given transmission interval. For example, in Figure \ref{fig:sub1} the entries $(3,1), (3,2), (1,3), (1,4), (1,5)$ are dark shaded, which means the first transmission vector at round 1, i.e. $\Bx(1)$, includes $A_3^1,B_3^1, C_1^1, D_1^1, E_1^1$; and $\CT(1)=[1:5]$. With $L=3$ antennas, each part can be nulled out at two users; and we have
\begin{equation}\label{eq:tx1}
    \begin{aligned}
        \Bx(1) = &A_3^1 \Bv_{\{1,3,4\}} + B_3^1 \Bv_{\{2,3,4\}} \\
            &+ C_1^1 \Bv_{\{1,2,3\}} + D_1^1 \Bv_{\{1,2,4\}} + E_1^1 \Bv_{\{1,2,5\}} \; . \\
    \end{aligned}
\end{equation}
Note that all superscripts are set to 1, as no data is transmitted prior to $\Bx(1)$. According to \eqref{eq:reception_model} and \eqref{eq:zeroforce_definition}, user 1 receives
\begin{equation}
\label{eq:first_transmission}
    \begin{aligned}
        y_1(1) = &A_3^1 \Bh_1^T \Bv_{\{1,3,4\}} +  \underline{C_1^1 \Bh_1^T \Bv_{\{1,2,3\}}} \\
        &+ \underline{D_1^1 \Bh_1^T \Bv_{\{1,2,4\}}} + \underline{E_1^1 \Bh_1^T\Bv_{\{1,2,5\}}} + w_1(1) \; .
    \end{aligned}
\end{equation}
From Example \ref{exmp:placement_matrix}, we know that $W_1^1 \in \CZ(1)$, $\forall W \in \CF$. Also, based to the system model, user 1 can estimate $\Bh_1^T \Bv_{\CR}$, $\forall \CR$. This means user 1 can reconstruct and remove the underlined terms from its received signal in \eqref{eq:first_transmission}; and finally decode $A_3^1$ interference-free. Similarly, users 2, 3, 4, 5 can decode $B_3^1$, $C_1^1$, $D_1^1$, $E_1^1$ respectively, resulting in DoF of $t+L = 5$ for the first transmission interval.
%This is on par with the first transmission vector created using $\BR_1$ and $\BC_1$, as discussed in Example \ref{exmp:trans_vectors_exmp}. In fact, Figure \ref{fig:graph_exmp_r1c1} graphically represents the four transmission vectors created by $\BR_1$ and $\BC_1$, while Figure \ref{fig:graph_exmp_r2c2} does the same for $\BR_2$ and $\BC_2$.

%\input{Figures/ICCExample-R1C1}

%\input{Figures/ICCExample-R2C2}

The next transmission vectors in round 1, i.e. $\Bx(2)$-$\Bx(4)$, are built by circular shift of $\Bx(1)$ elements over the non-shaded cells of the grid, in two perpendicular directions. Specifically, the first two terms of $\Bx(1)$ are shifted vertically, while the other three terms are shifted horizontally. This procedure is depicted in Figures \ref{fig:sub2}-\ref{fig:sub4}. So $\Bx(2)$ is built as
\begin{equation}
    \begin{aligned}
        \Bx(2) = &A_4^1 \Bv_{\{1,4,5\}} + B_4^1 \Bv_{\{2,4,5\}} \\
            &+ D_1^2 \Bv_{\{1,2,4\}} + E_1^2 \Bv_{\{1,2,5\}} + F_1^1 \Bv_{\{1,2,6\}} \; , \\
    \end{aligned}
\end{equation}
where the superscripts for $D_1$ and $E_1$ are updated to 2, as $D_1^1$ and $E_1^1$ were transmitted by $\Bx(1)$. Similarly, $\Bx(3)$ and $\Bx(4)$ are built as
\begin{equation}
    \begin{aligned}
        \Bx(3) = &A_5^1 \Bv_{\{1,5,6\}} + B_5^1 \Bv_{\{2,5,6\}} \\
            &+ E_1^3 \Bv_{\{1,2,5\}} + F_1^2 \Bv_{\{1,2,6\}} + C_1^2 \Bv_{\{1,2,3\}} \; , \\
        \Bx(4) = &A_2^1 \Bv_{\{1,2,3\}} + B_6^1 \Bv_{\{1,2,6\}} \\
            &+ F_1^3 \Bv_{\{1,2,6\}} + C_1^3 \Bv_{\{1,2,3\}} + D_1^3 \Bv_{\{1,2,4\}} \; .
    \end{aligned}
\end{equation}
% respectively based on Figures \ref{fig:sub3} and \ref{fig:sub4}.
% Altogether, $\Bx(1)$-$\Bx(4)$ constitute the first \textit{transmission round}.

The second transmission round includes $\Bx(5)$-$\Bx(8)$, which are built by diagonal shift (simultaneous circular shift of one unit to the right and down)
%Circular increment is formally defined in Section \ref{section:delivery_prime_matrix}.
of $\Bx(1)$-$\Bx(4)$; as shown in Figure~\ref{fig:graph_exmp_r2c2}. Similarly, the third round is built by diagonal shift of $\Bx(5)$-$\Bx(8)$, and this procedure continues until $\Bx(21)$-$\Bx(24)$ are built by diagonal shift of the transmission vectors of the previous round. In total, $6 \times 4 = 24$ transmission intervals are required and each missing part will appear $2+3 = 5$ times; resulting in total subpacketization requirement of $6 \times 5 = 30$.
%\footnote{In this example, the required subpacketization is larger than the scheme of \cite{shariatpanahi2016multi}. The intention is to show how the linear growth in subpacketization is achieved. Comparison with other schemes is provided in Section \ref{Section:performance_analysis}.}

For a general network setup with parameters $K, t, L$, in a single round we have $K-t$ transmission vectors, and each new round is built by diagonal shift of transmission vectors in the previous round. There exist a total number of $K$ rounds, resulting in $S = K \times (K-t)$ total transmission intervals; and the required subpacketization is $K \times (t+L)$.
%The algorithmic procedure for this delivery scheme is discussed in subsequent sections.

%Taking a closer look at Figures \ref{fig:graph_exmp_r1c1} and \ref{fig:graph_exmp_r2c2}, it can be seen that the delivery algorithm works based on two circular shift operations over the table, in vertical and horizontal directions. The respective shift areas are distinguished by darker lines in the tables. In fact, PD matrix generation algorithms are designed such that for each pair of resulting $\BR_k$ and $\BC_k$ matrices, this circular shift property is achieved by picking file part and user indices from $\BR_k$ and $\BC_k$, respectively.



==> LiteratureReview.tex <==

\subsubsection{Coded caching}
The original coded caching scheme, proposed by Maddah-Ali and Niesen in~\cite{maddah2014fundamental}, considers a normalized symmetric broadcast channel connecting a single server (transmitter) to $K$ users (receivers). The server hosts a library of $ N $ equal-sized files, and each user has a cache memory with the capacity to store $ M $ files. System operation is assumed to consist of two distinct phases: cache placement and content delivery. During the cache placement phase, which occurs during the off-peak hours, the users' cache memories are filled with (parts of) the files in the library. Then, at the content delivery phase, which happens at the peak hours, multicasting opportunities made available by the placement phase are used to serve multiple users simultaneously. The meticulous design of the placement phase, together with the use of coded multicasting in the delivery phase, allows the scheme to increase the known achievable sum \textit{Degrees of Freedom} (DoF) of the channel from $1$ to $t+1$, where $t\coloneqq \frac{KM}{N}$ is the coded caching gain. In a nutshell, each transmission in the delivery phase includes the superposition of messages intended for a distinct subset of $t+1$ users. Each user in the subset can then use its locally cached content, to remove the interfering messages intended for other users and obtain its desired message interference-free. This scheme is later proven to be optimal within a multiplicative gap of 2 in~\cite{yu2018characterizing}, and exactly optimal under the assumption of uncoded cache placement in~\cite{wan2016optimality,yu2017exact}. It is also extended in various directions, such as decentralized, hierarchical and device to device (D2D) assisted coded caching \cite{maddah2015decentralized,karamchandani2016hierarchical,ji2015fundamental}.

\subsubsection{Multi-antenna coded caching and finite-SNR analysis}
For a setting where the cache-aided users are connected through a linear network to $L$ transmitting servers, the work in~\cite{shariatpanahi2016multi} proposes a scheme that achieves a sum-DoF of $t+L$. Under the assumption of uncoded cache placement, this DoF is recently proven in~\cite{lampiris2018resolving} to be optimal from the one-shot linear sum-DoF sense. Following the same concept, the implementation of coded caching techniques in multi-antenna wireless networks with zero-forcing (ZF) precoders is later studied in~\cite{shariatpanahi2017multi,shariatpanahi2018physical}. However, while the proposed solutions perform well in the high-SNR regime, their performances are not satisfactory in low-SNR communications. For the low-SNR regime, the performance is improved in~\cite{tolli2018multicast} by replacing ZF precoders with optimized beamformers. As a result, the inter-stream interference is controlled instead of being nulled out, without losing the multicasting opportunities provided by coded caching. Later, in~\cite{tolli2017multi}, novel methods are introduced to reduce the optimized beamformer design complexity. These methods are based on two design parameters $ \alpha$ and $ \beta$, which control the spatial multiplexing gain and the multiple-access channel (MAC) size at each user. It is shown that choosing $\alpha$ to be smaller than its maximum value of $L$ not only reduces the beamformer design complexity but also enables an improved beamforming gain, which boosts the performance in the low-SNR regime. Controlling the spatial multiplexing gain is also considered in~\cite{lampiris2019bridgingb}, where numerical simulations are used to find the multiplexing gain resulting in the best performance. It is shown that the optimal multiplexing gain depends on various network parameters, including the coded caching gain $t$. From another perspective, by limiting the number of messages received by a user in each time slot, the work in~\cite{zhao2020multi} proposes a new scheme that aims to reduce the complexity while providing a satisfactory rate. Other works in the same line of research are~\cite{shariatpanahi2018multi,lampiris2019fundamental,bergel2018cache}. Although the numerical simulations show that the discussed schemes achieve promising performances, they all require large subpacketization values, making them infeasible even for a moderate number of users in the network. 

\subsubsection{Subpacketization bottleneck}
For coded caching schemes to work properly, one needs to split every library file into several smaller parts. The number of these smaller parts is known as \textit{subpacketization} in the literature. Unfortunately, many coded caching schemes require subpacketization values that grow exponentially, with the user count $K$ (for fixed $\frac{M}{N}$). For example, the original coded caching scheme in~\cite{maddah2014fundamental} has a subpacketization requirement of $\binom{K}{t}$; and for the multi-antenna scheme in~\cite{shariatpanahi2018physical}, the subpacketization requirement is $\binom{K}{t} \binom{K-t-1}{L-1}$, where $L$ is the number of transmitting antennas. Consequently, reducing subpacketization (without considerably damaging the DoF) has been studied in the literature, both for single- and multi-antenna setups.

In the context of single-antenna setups, in~\cite{shanmugam2016finite}, it is shown that decentralized schemes need exponential subpacketization to achieve any sub-linear coded caching gain, for constant $\frac{M}{N}$ as $K \rightarrow \infty$. In~\cite{yan2017placement} placement delivery array (PDA) is presented as a systematic approach to reducing subpacketization in centralized schemes. It is shown that the original scheme of~\cite{maddah2014fundamental} is a PDA-driven scheme; and is optimal among one symmetric class of schemes known as $g$-regular PDA. 
Following~\cite{yan2017placement}, in~\cite{yan2018placement} it is shown that for a constant rate, a PDA resulting in linear subpacketization does not exist. In~\cite{shangguan2018centralized}, for fixed rate and $\frac{M}{N}$, a new scheme with sub-exponential subpacketization is proposed. In~\cite{shanmugam2017coded} Ruzsa-Szem{\'e}redi graphs are used to design coded caching schemes with linear subpacketization as $K \rightarrow \infty$, but with non-constant rate.

For the multi-antenna setups, fewer results are available on subpacketization reduction. A notable work on this topic is~\cite{lampiris2018adding}, in which it is shown that if $\frac{K}{L}$ and $\frac{t}{L}$ are both integers, the DoF of $t+L$ is achievable with the reduced subpacketization of~$\binom{K/L}{t/L}$. Interestingly, this subpacketization value is even smaller than the single-antenna scheme of~\cite{maddah2014fundamental}, enabling a multiplicative DoF boost when the subpacketization is upper bounded due to practical limitations.
Unfortunately though, the scheme of~\cite{lampiris2018adding} suffers DoF loss (and also increased subpacketization), if either $\frac{K}{L}$ or $\frac{t}{L}$ is non-integer. Especially, DoF is reduced
by a multiplicative factor (gap), that is bounded by 2 when $L > t$, and by $\frac{3}{2}$ when $L < t$. For the same setting, the recent work in \cite{mohajer2020miso} proposes a DOF-optimal scheme which requires a subpacketization level that equals the one of Maddah-Ali and Niesen in \cite{maddah2014fundamental} for the shared-link scenario. This reduction in subpacketization also comes with a reduction in transmission and decoding complexity compared to the multi-server scheme with optimized beamformers in~\cite{tolli2017multi}. However, the scheme suffers a small reduction in performance compared to \cite{tolli2017multi}, and its subpacketization requirement is still exponential with $ K$. As a result, it is also not practical for real networks with a large number of users.

The main idea behind the work in~\cite{lampiris2018adding} is to partition the set of all users into $\frac{K}{L}$ \textit{groups}, such that each group contains $L$ users with the same cache contents. This user-grouping idea can also be interpreted as a shared-cache setting~\cite{shanmugam2016finite}, which has been used to represent more complex networks (and as a tool for subpacketization reduction in case the users have dedicated caches). Interestingly, while for single-antenna setups it is shown that DoF loss is inevitable for a shared-cache setting~\cite{parrinello2019fundamental}, in~\cite{lampiris2018adding} it is shown that for multi-antenna setups there can be no reduction in the maximum achievable DoF, if users in the same group are forced to cache the same content.

In~\cite{salehi2019subpacketization} it is shown that subpacketization can be traded-off with the performance, and a new approach is introduced for selecting subpacketization flexibly. However, the results are limited to the specific case of $K = t+L$. In~\cite{lampiris2019bridging} joint reduction of channel state information (CSI) and subpacketization requirements is considered, and it shown that subpacketization of $L_c \binom{K_c}{t}$ is achievable, where $L_c \coloneqq \frac{L+t}{t+1}$ and $K_c \coloneqq \frac{K}{L_c}$. However, the proposed scheme requires both $L_c$ and $K_c$ to be integers, making it applicable to a narrow set of network parameters. Moreover, it results in a DoF loss by a factor of $(1-\frac{t}{K})$.

\subsection{Our Contribution}
In this paper, motivated by the current trend of deploying antenna arrays at the base stations, we study a cache-aided multiple-input single-output (MISO) broadcast channel with $L$ antennas at the transmitter side. Assuming the coded caching gain is $t \coloneqq \frac{KM}{N}$ and $t$ is not larger than $L$, we set the spatial DoF to be $t \le \alpha \le L$. Although the $\alpha \le L$ assumption reduces the maximum achievable sum-DoF from (the optimal value of) $t+L$ to $t+\alpha$, in~\cite{tolli2017multi} it is shown that, in the low-to-medium SNR regime, it can improve the performance as it allows to compensate for the user with the worst channel condition by providing an improved beamforming gain. In our setup, we consider $\alpha$ is a design parameter that can be tuned to control the subpacketization (and complexity) and, at the same time, to adjust the performance at the low- and mid-SNR regimes.

We introduce an entirely new high-performance low-subpacketization coded caching scheme, applicable to networks with large transmitting antenna arrays in which $\alpha \ge t$. The proposed scheme, which we call \textit{cyclic caching}, is based on the circular shifting of vectors over a tabular structure and requires much smaller subpacketization values than state of the art. 
Crucially, cyclic caching achieves the sum-DoF of $t+\alpha$ with the subpacketization requirement of only $\frac{K(t+\alpha)}{\phi_{K,t,\alpha}^2}$, where $\phi_{K,t,\alpha} = gcd(K,t,\alpha)$ and $gcd$ denotes the greatest common divisor. This subpacketization requirement not only grows linearly with the network size (or quadratic, based on how the parameters scale with each other) but can also be effectively controlled by changing the $\alpha$ (and $K$, as will be discussed later) parameter. 
On the other hand, cyclic caching also eliminates the requirement of multicasting, thus interestingly enabling optimized MMSE (minimum mean square error) type beamformers to be designed with much less computational complexity. Optimized beamformers allow an interplay between cache cancellation, nulling out, and controlling the interference, thus improving the performance considerably at low- and mid-SNR communications. In the end, the work yields a low-subpacketization multi-antenna coded caching solution that provides an excellent performance at the finite-SNR regime and can be efficiently applied to networks with a large number of users.

%The proposed scheme not only requires much smaller subpacketization values compared with the state of the art but also benefits from an underlying cache-aided interference cancellation mechanism that enables efficient optimized MMSE (minimum min-square error) type beamformers to be applied with low computational complexity. This enables the performance of the proposed scheme to be superior at the low- and mid-SNR regime, compared with the case zero-forcing beamformers are used to completely remove the inter-stream interference. In other words, our scheme enables an interplay between cache cancellation and interference suppression, which results in a highly efficient low-subpacketization coded caching scheme with an appropriate performance at the finite-SNR regime.

%To put it in more details, the cyclic scheme presented in this paper achieves the sum-DoF of $t+\alpha$ during each transmission, with a subpacketization requirement of only $S=\frac{K(t+L)}{\phi^2}$, where $\phi=gcd(K,t,\alpha)$ and $gcd$ denotes the greatest common divisor.





%We provide a novel coded caching scheme for the proposed setup, with low complexity in terms of both subpacketization and beamforming design. The new scheme achieves the optimal sum-DoF of $t+\alpha$, with a subpacketization requirement of only $S=\frac{K(t+L)}{\phi^2}$, where $\phi=gcd(K,t,\alpha)$ and $gcd$ denotes the greatest common divisor. This makes our scheme the first in the literature to achieve the optimal sum-DoF with a slowly-increasing subpacketization, enabling it to be applicable in networks with a large number of users. The scalability of our scheme is also driven by the fact that each user receives at most one single message after every transmission, thus not requiring successive interference cancellation (SIC) receivers unlike some previously proposed schemes such as~\cite{shariatpanahi2016multi,tolli2017multi}.

%Interestingly, the underlying cache-aided interference cancellation mechanism of the proposed scheme not only eliminates the need for SIC receivers but also enables the data delivery to rely entirely on unicasting. In other words, each user receives at most one single message after every transmission, and at the same time, each data part sent during any transmission is intended for one user only. This enables the optimized MMSE-type beamformer design problem to be easily solvable using uplink-downlink duality. While zero-forcing beamformers completely null out the interference at unwanted users, optimized beamformers enable an interplay between nulling out and controlling the interference, improving the performance considerably at the finite-SNR regime~\cite{tolli2017multi}. Together with the low-subpacketization requirement, the simple applicability of optimized beamformers results in a highly efficient, scalable multi-antenna coded caching scheme with an appropriate performance at the finite-SNR regime.

%\textcolor{blue}{We should remove ZF} Inspired by the works~\cite{tolli2017multi,salehi2019beamformer}, we study both zero-forcing (ZF) and optimized (MMSE-like) beamforming strategies. While in the ZF strategy the interference is completely nulled out at unwanted users, in the optimized strategy the interference is allowed in a controlled way. While ZF beamformers are much simpler to design, it is well-known that they cause a considerable performance decay at the low-SNR regime. However, as studied in~\cite{tolli2017multi}, this can be addressed by selecting a smaller $\alpha$ value. Interestingly, in our proposed coded caching scheme, controlling $\alpha$ not only enables high-performance, simple beamformers to be designed, but it also allows smaller subpacketization to be achieved, by adjusting the $\phi$ value. Overall, these nice properties make our proposed scheme feasible for implementation in practical, large networks. \textcolor{blue}{Petros: We can accentuate the fact that while in the DOf regime interference is either cached out or nulled out in its entirety, this work here explores the interplay between caching out, nulling out an controlling interference, where this interplay varies as a function of SNR.}

%In this paper, motivated by the current trend of deploying large antenna arrays at the base stations and by the relatively limited memory at each user terminal, we study a cache-aided MISO broadcast channel and we focus only on networks with $L\geq t$.

%We propose a novel multi-antenna coded caching scheme which has a low-complexity both in terms of subpacketization and beamforming design. We show that the new scheme achieves the optimal sum DoF of $t+L$ with a subpacketization requirement of only $S=\frac{K(t+L)}{\phi_L^2}$, with $\phi_L=gcd(K,L,t)$. 

%This makes our scheme the first in the literature to achieve the optimal DoF with a slowly-increasing subpacketization with the network size, making the scheme salable to be applied in networks with a large set of users. The scalability of our scheme is also made possible by the fact that each users receives only a single message at a time, thus not requiring successive interference cancellation (SIC) receivers, unlike other previously proposed schemes such us \cite{shariatpanahi2016multi,tolli2017multi}. 

%Inspired by the works \cite{tolli2017multi,salehi2019beamformer}, in this paper we present 2 different beamforming strategies: the ZF beamforming and the optimized (MMSE-like) beamforming. As in cite{}, the first completely nulls interference at unwanted users and optimally allocates the power among the parallel streams, while the second strategy allows some interference in order to better balance the impact of noise and inter-stream interference. It is well known that ZF heavily suffers in the low SNR regime, however we will show that reducing the size of the user subset served during a given time interval from $t+L$ to $t+\alpha$ ($\alpha\leq L$), as it has been done in \cite{tolli2017multi}, allows to compensate for the worst-user and simultaneously achieve multiplexing gain, thus providing a good performance in the low-to-medium SNR regime at the expenses of a reduced sum DoF. At the same time, this reduction in DoF can be very beneficial in terms of subpacketization, which can be further dropped down to $S=\frac{K(t+\alpha)}{\phi_{\alpha}^2}$, with $\phi_{\alpha}=gcd(K,t,\alpha)$. Overall, the structure of the novel scheme which intrinsicly does not require SIC receivers, together with the flexibility provided by parameter $\alpha$, result in a scheme that achieves good performance both in a broad range of the SNR spectrum and at the same time, requires low complexity in terms of precoder design and subpacketization. Overall, these interesting features make the new scheme feasible for implementation in practical, large networks.


\subsection{Structure and Notation}
In this paper, we use $[K]$ to denote the set $\{1,2,...,K\}$ and $[i:j]$ to represent the vector $[i \; i\!+\!\!1 \; ... \; j]$. Boldface upper- and lower-case letters denote matrices and vectors, respectively. $\BV[i,j]$ refers to the element at the $i$-th row and $j$-th column of matrix $\BV$, and $\Bw[i]$ is the $i$-th element in vector $\Bw$.
Moreover, $\Bw=[\Bu;\Bv]$ means $\Bw$ is formed by the concatenation of two vectors $\Bu$ and $\Bv$. Sets are denoted by calligraphic letters. For two sets $\CA$ and $\CB$, $\CA \backslash \CB$ is the set of elements in $\CA$ that are not in $\CB$, and $|\CA|$ represents the number of elements in $\CA$.

The rest of the paper is organized as follows. In Section~\ref{section:sys_model} we provide the system model. Section~\ref{section:ICCPaper} is devoted to introducing the new cyclic caching scheme, where we first show that the subpacketization of $K(t+\alpha)$ is possible with sum-DoF of $t+\alpha$, for any network in which $\alpha \ge t$; and then show that the subpacketization can be further reduced by a factor of $\phi_{K,t,\alpha}^2$. Moreover, we show that the proposed scheme follows a simple graphical representation, based on the cyclic shifting of two vectors over a tabular structure. In Section~\ref{section:sim_results}, we analyze the complexity and simulate the performance of the proposed scheme. Finally, in Section~\ref{section:conclusion}, we conclude the paper.

